Formalizing Representation Theorems for a Logical Framework with Rewriting

Representation theorems for formal systems often take the form of an inductive translation that satisfies certain invariants, which are proved inductively. Theory morphisms and logical relations are common patterns of such inductive constructions. They allow representing the translation and the proofs of the invariants as a set of translation rules, corresponding to the cases of the inductions. Importantly, establishing the invariants is reduced to checking a finite set of, typically decidable, statements. Therefore, in a framework supporting theory morphisms and logical relations, translations that fit one of these patterns become much easier to formalize and to verify. The lambdaPi-calculus modulo rewriting is a logical framework designed for representing and translating between formal systems that has previously not systematically supported such patterns. In this paper, we extend it with theory morphisms and logical relations. We apply these to define and verify invariants for a number of translations between formal systems. In doing so, we identify some best practices that enable us to obtain elegant novel formalizations of some challenging translations, in particular sort-erasure translations from sorted to unsorted languages.

==> embeddings.tex <==


We have seen that theory morphisms may erase some information, that may be retrieved using logical relations. However, for some translations between theories, the invariants are critical, meaning that the theory morphism cannot work in their absence. This is for example the case when we want to translate natural numbers $\El ~\nat$ into integers $\El ~\int$, because the fact that natural numbers are non-negative integers is essential. 

One approach is to consider dependent sums and pairs, so that the invariant is directly inserted into the translation. For instance, we could map $\El ~\nat$ to $\Sigma x : \El ~\int. ~\Prf ~(x \geq 0)$ to ensure that natural numbers are mapped to non-negative integers. Lax theory morphisms~\cite{rabe:lax:14} solve this issue, as they allow to pair the translation and the proofs of its invariants. However, lax theory morphisms introduce dependent pairs---which are not in the syntax of \lf and \lpr---and are not homomorphically defined---meaning that the translation cannot be simply defined by parameters on the constants like theory morphisms and logical relations are.

In this section, we propose theory embeddings, a new translation template in which the morphism and the proofs of its invariants are mutually defined by induction. In that respect, this template corresponds to a theory morphism where dependent sums have been uncurried. Satisfactorily, theory embeddings are syntactic translations, based on the parameters chosen for each constant of the source theory.




\subsection{Motivating Example: Natural Numbers and Integers}


An illustrative example of theory embedding is the translation from natural numbers to integers. 
The theory morphism template cannot be used, because the invariant---stating that the integers representing natural numbers must be non-negative---is essential to the translation.

The theory of natural numbers and the theory of integers both rely on the encoding of the Calculus of Constructions in \lpr~\cite{theoryU}. 
The notions of propositions and proofs are encoded using the following constants. 
%%
\begin{flalign*}
&\Set : \Type & &\o : \Set & &\El : \Set \ra \Type & &\Prf : \El ~\o \ra \Type  
\end{flalign*}
%%%
The symbols $\arrd$, $\impd$, $\pi$ and $\fa$ are used to quantify over object terms and proof terms inside object terms and proof terms.
%%
\begin{flalign*}
&\arrd : \Pi x : \Set. ~(\El ~x \ra \Set) \ra \Set & &\El ~(x \arrd y) \lra \Pi z : \El ~x. ~\El ~(y ~z) \\
&\impd : \Pi x : \El ~\o. ~(\Prf ~x \ra \El ~\o) \ra \El ~\o & &\Prf ~(x \impd y) \lra \Pi z : \Prf ~x. ~\Prf ~(y ~z) \\
&\pi : \Pi x : \El ~\o. ~(\Prf ~x \ra \Set) \ra \Set & &\El ~(\pi ~x ~y) \lra \Pi z : \Prf ~x. ~\El ~(y ~z) \\
&\fa : \Pi x : \Set. ~(\El ~x \ra \El ~\o) \ra \El ~\o & &\Prf ~(\fa ~x ~y) \lra \Pi z : \El ~x. ~\Prf ~(y ~z) 
\end{flalign*}
%%%
We define the sort $\nat$ for natural numbers, with the two constructors $0$ and $\succ$. The relation $\geq$ is reflexive and transitive, with $\succ ~x \geq x$.
%%%
\begin{flalign*}
&\nat : \Set & \\
&0 : \El ~\nat & \\
&\succ : \El ~\nat \ra \El ~\nat & \\
&\geq ~: \El ~\nat \ra \El ~\nat \ra \El ~\o & \\
&\ax_1 : \Pi x : \El ~\nat. ~\Prf ~(x \geq x) & \\
&\ax_2 : \Pi x : \El ~\nat. ~\Prf ~(\succ ~x \geq x) & \\
&\ax_3 : \Pi x,y,z : \El ~\nat. ~\Prf ~(x \geq y) \ra \Prf ~(y \geq z) \ra \Prf ~(x \geq z) & 
\end{flalign*}
%%%
The theory of integers contains the same constants, but with $\int$ instead of $\nat$. The theory of natural numbers and the theory of integers differ by their induction principle. The induction principle on natural numbers is
%%% 
\[
\begin{array}{ll}
\rec : &\Pi P : \El ~\nat \ra \El ~\o. ~\Prf ~(P ~0) \ra \\
 &[\Pi x : \El ~\nat. ~\Prf ~(P ~x) \ra \Prf ~(P ~(\succ ~x))] \ra \\
 &\Pi x : \El ~\nat. ~\Prf ~(P ~x) 
\end{array}
\]
%%%
while the induction principle on integers is 
%%%
\[
\begin{array}{ll}
\rec : &\Pi x_0 : \El ~\int. ~\Pi P : \El ~\int \ra \El ~\o. ~\Prf ~(P ~x_0) \ra \\
 &[\Pi x : \El ~\int. ~\Prf ~(x \geq x_0) \ra \Prf ~(P ~x) \ra \Prf ~(P ~(\succ ~x))] \ra \\
 &\Pi x : \El ~\int. ~\Prf ~(x \geq x_0) \ra \Prf ~(P ~x) 
\end{array}
\]
%%%
In the theory of natural numbers, we can easily prove the theorem $\Pi x : \El ~\nat. ~\Prf ~(\succ ~x \geq 0)$. We cannot use a theory morphism mapping natural numbers to integers, because we would obtain the theorem $\Pi x : \El ~\int. ~\Prf ~(\succ ~x \geq 0)$, which is obviously false. We need to insert a predicate asserting that $x$ is non-negative directly in the translation.




\subsection{Formal Definition}


Theory embeddings are composed of two translations, $\m$ and $\r$, that are mutually defined by induction. The translation $\r$ works exactly like logical relations. On the contrary, the translation $\m$ is different from theory morphisms, as $\m$ depends on $\r$, while $\mor$ is independent from $\lr$. The translation $\m$ ensures that crucial invariants of the source theory are preserved in the target theory thanks to its dependence on $\r$. 

In particular, $\m(M ~N)$ is given by $\m(M) ~\m(N) ~\r(N)$, where $\r(N)$ is a witness asserting that $\m(N)$ indeed satisfies the invariant. Similarly, $\m(\lambda x : A. ~M)$ is given by $\lambda x : \m(A). ~\lambda x^* : \r(A) ~x. ~\m(M)$, because we ask a witness $x^*$ that $x$ satisfies the predicate $\r(A)$.


\begin{definition}
The mappings $\m$ and $\r$ defined inductively and mutually from a set pf parameters $\m_c$, $\m_a$, $\r_c$ and $r_a$ by
\[
\begin{array}{lll}
\m(x) &= &x \\
\m(c) &= &\m_c \\
\m(a) &= &\m_a \\
\m(M ~N) &= &\m(M) ~\m(N) ~\r(N) \\
\m(A ~M) &= &\m(A) ~\m(M) ~\r(M) \\
\m(\lambda x : A. ~M) &= &\lambda x : \m(A). ~\lambda x^* : \r(A) ~x. ~\m(M) \\
\m(\lambda x : A. ~B) &= &\lambda x : \m(A). ~\lambda x^* : \r(A) ~x. ~\m(B)  \\
\m(\Pi x : A. ~B) &= &\Pi x : \m(A). ~\Pi x^* : \r(A) ~x. ~\m(B) \\
\m(\Pi x : A. ~K) &= &\Pi x : \m(A). ~\Pi x^* : \r(A) ~x. ~\m(K) \\
\m(\Type) &= &\Type \\
\m(\Kind) &= &\Kind \\
&&\\
\r(x) &= &x^* \\
\r(c) &= &\r_c \\
\r(a) &= &\r_a \\
\r(M ~N) &= &\r(M) ~\m(N) ~\r(N) \\
\r(A ~M) &= &\r(A) ~\m(M) ~\r(M) \\
\r(\lambda x : A. ~M) &= &\lambda x : \m(A). ~\lambda x^* : \r(A) ~x. ~\r(M) \\
\r(\lambda x : A. ~B) &= &\lambda x : \m(A). ~\lambda x^* : \r(A) ~x. ~\r(B)  \\
\r(\Pi x : A. ~B) &= &\lambda f : \m(\Pi x : A. ~B). ~\Pi x : \m(A). ~\Pi x^* : \r(A) ~x. ~\r(B) ~(f ~x ~x^*) \\
\r^{R}(\Pi x : A. ~K) &= &\Pi x : \m(A). ~\Pi x^* : \r(A) ~x. ~\r^{R ~x}(K) \\
\r^{R}(\Type) &= &\m(R) \ra \Type \\
\r(\Kind) &= &\Kind 
\end{array}
\]
are a theory embedding of $\S$ into $\T$ when:
\begin{enumerate}
\item for every constant $c : A \in \S$, there exist terms $\m_c$ and $\r_c$ such that $\vdash_\T \m_c : \m(A)$ and $\vdash_\T \r_c : \r(A) ~\m_c$,
\item for every constant $a : K \in \S$, there exist terms $\m_a$ and $\r_a$ such that $\vdash_\T \m_a : \m(K)$ and $\vdash_\T \r_a : \r^{a}(K)$,
\item for every rewrite rule $\ell \lra r \in \S$, we have $\m(\ell) \equiv_{\beta\Sigma} \m(r)$ and $\r(\ell) \equiv_{\beta\Sigma} \r(r)$ in $\T$.
\end{enumerate}
\end{definition}

The conditions for building a theory embedding of the source theory into the target theory combines the conditions of theory morphisms and logical relations. 

For any variable $x$ that occurs in a term $t$, both variables $x$ and $x^*$ occur in its translations $\m(t)$ and $\r(t)$. In that respect, we extend theory embeddings to contexts using a single translation $\mr$, defined inductively by
\[
\begin{array}{lll}
\mr(\varnothing) &= &\varnothing \\
\mr(\Gamma, x : A) &= &\mr(\Gamma), x : \m(A), x^* : r(A) ~x
\end{array}
\]
which duplicates each variable. 






\subsection{Embedding Theorem}


The Embedding theorem corresponds to both the Representation theorem for theory morphisms and to the Abstraction theorem for logical relations. 



\begin{theorem}[Embedding]
\label{thm_embedding}
Let $\m$ and $\r$ be a theory embedding of $\S$ into $\T$.
\begin{enumerate}
\item If $\vdash_\S \Gamma$ then $\vdash_\T \mr(\Gamma)$.
\item If $\Gamma \vdash_\S M : A$ then $\mr(\Gamma) \vdash_\T \m(M) : \m(A)$.
\item If $\Gamma \vdash_\S A : K$ then $\mr(\Gamma) \vdash_\T \m(A) : \m(K)$.
\item If $\Gamma \vdash_\S K : \Kind$ then $\mr(\Gamma) \vdash_\T \m(K) : \Kind$.
\item If $\Gamma \vdash_\S M : A$ and $\Gamma \vdash_\S A : \Type$, then $\mr(\Gamma) \vdash_\T \r(M) : \r(A) ~\m(M)$.
\item If $\Gamma \vdash_\S A : K$ and $\Gamma \vdash_\S K : \Kind$, then $\mr(\Gamma) \vdash_\T \r(A) : \r^{A}(K)$.
\item If $\Gamma \vdash_\S K : \Kind$ and $\Gamma \vdash_\S A : K$, then we have $\mr(\Gamma) \vdash_\T \r^{A}(K) : \Kind$.
\end{enumerate}
\end{theorem}


We have seen that theory embeddings are extended to contexts using a single translation $\mr$. It follows that theory embeddings are extended to substitutions using
$$\mr([x_1 \leftarrow N_1, \ldots, x_n \leftarrow N_n]) = [x_1 \leftarrow \m(N_1), x_1^* \leftarrow \r(N_1), \ldots, x_n \leftarrow \m(N_n), x_n^* \leftarrow \r(N_n)]$$
where the number of assigned variables in the translated substitutions is twice the number of assigned variables in the original substitution.


\begin{lemma}[Substitution]
\label{prop_subst_mr}
Let $\m$ and $\r$ be a theory embedding of $\S$ into $\T$, and $\theta$ be a substitution.
\begin{enumerate}
\item $\m(M\theta) = \m(M)\mr(\theta)$
\item $\r(M\theta) = \r(M)\mr(\theta)$
\item $\m(A\theta) = \m(A)\mr(\theta)$
\item $\r(A\theta) = \r(A)\mr(\theta)$
\item $\m(K\theta) = \m(K)\mr(\theta)$
\item $\r^{A\theta}(K\theta) = \r^{A}(K)\mr(\theta)$
\end{enumerate}
\end{lemma}


\begin{lemma}[Conversion]
\label{prop_conv_mr}
Let $\m$ and $\r$ be a theory embedding of $\S$ into $\T$.
\begin{enumerate}
\item If $A \equiv_{\beta\R} B$ in $\S$ then $\m(A) \equiv_{\beta\R} \m(B)$ in $\T$.
\item If $A \equiv_{\beta\R} B$ in $\S$ then $\r(A) \equiv_{\beta\R} \r(B)$ in $\T$.
\item If $K \equiv_{\beta\R} K'$ in $\S$ then $\m(K) \equiv_{\beta\R} \m(K')$ in $\T$.
\item If $K \equiv_{\beta\R} K'$ in $\S$ then $\r^{R}(K) \equiv_{\beta\R} \r^{R}(K')$ in $\T$.
\end{enumerate}
\end{lemma}



\begin{proof}[Proof of \Cref{thm_embedding}]
We proceed by induction on the derivations.
\begin{itemize}
\item \underline{\textbf{Empty}}: Since $\mr(\varnothing) = \varnothing$, we derive $\vdash_\T \mr(\varnothing)$ using \textsc{Empty}.


\item \underline{\textbf{Decl}}: By induction, we get $\vdash_\T \mr(\Gamma)$, and $\mr(\Gamma) \vdash_\T \m(A) : \Type$, and $\mr(\Gamma) \vdash_\T \r(A) : \m(A) \ra \Type$. We conclude $\vdash_\T \mr(\Gamma), x : \m(A), x^* : \r(A) ~x$ using \textsc{Decl}.


\item \underline{\textbf{Sort}}: Suppose that $\Gamma \vdash_\S A : \Type$. By induction, we get $\vdash_\T \mr(\Gamma)$ and $\mr(\Gamma) \vdash_\T \m(A) : \Type$. We obtain $\mr(\Gamma) \vdash_\T \Type : \Kind$ and $\mr(\Gamma) \vdash_\T \m(A) \ra \Type : \Kind$.


\item \underline{\textbf{Const-Obj}}: By induction, we get $\vdash_\T \mr(\Gamma)$. Since $c : A \in \T$, we have $\vdash_\T \m_c : \m(A)$ and $\vdash_\T \r_c : \r(A) ~\m_c$. By weakening, we derive $\mr(\Gamma) \vdash_\T \m_c : \m(A)$ and $\mr(\Gamma) \vdash_\T \r_c : \r(A) ~\m_c$.


\item \underline{\textbf{Const-Type}}: By induction, we get $\vdash_\T \mr(\Gamma)$. Since $a : K \in \T$, we have $\vdash_\T \m_a : \m(K)$ and $\vdash_\T \r_a : \r^{a}(K)$. By weakening, we derive $\mr(\Gamma) \vdash_\T \m_a : \m(K)$ and $\mr(\Gamma) \vdash_\T \r_a : \r^{a}(K)$.


\item \underline{\textbf{Var}}: By induction, we get $\vdash_\T \mr(\Gamma)$. Since $x : A \in \Gamma$, we have $x : \m(A) \in \mr(\Gamma)$ and $x^* : \r(A) ~x \in \mr(\Gamma)$. We obtain $\mr(\Gamma) \vdash_\T x : \m(A)$ and $\mr(\Gamma) \vdash_\T x^* : \r(A) ~x$ using \textsc{Var}.


\item \underline{\textbf{Prod-Type}}: By induction, we get $\mr(\Gamma) \vdash_\T \m(A) : \Type$, and $\mr(\Gamma) \vdash_\T \r(A) : \m(A) \ra \Type$, and $\mr(\Gamma), x : \m(A), x^* : \r(A) ~x \vdash_\T \m(B) : \Type$. We obtain $\mr(\Gamma) \vdash_\T \Pi x : \m(A). ~\Pi x^* : \r(A) ~x. ~\m(B) : \Type$. 

By induction, we get $\mr(\Gamma), x : \m(A), x^* : \r(A) ~x \vdash_\T \r(B) : \m(B) \ra \Type$. By weakening, we derive $\mr(\Gamma), f : \m(\Pi x : A. ~B), x : \m(A), x^* : \r(A) ~x \vdash_\T \r(B) : \m(B) \ra \Type$. Since $\mr(\Gamma), f : \r(\Pi x : A. ~B), x : \m(A), x^* : \r(A) ~x \vdash_\T \r(B) ~(f ~x ~x^*) : \Type$, we obtain $\mr(\Gamma) \vdash_\T \lambda f : \m(\Pi x : A. ~B). ~\Pi x : \m(A). ~\Pi x^* : \r(A) ~x. ~\r(B) ~(f ~x ~x^*) : \m(\Pi x : A. ~B) \ra \Type$.


\item \underline{\textbf{Prod-Kind}}: By induction, we get $\mr(\Gamma) \vdash_\T \m(A) : \Type$, and $\mr(\Gamma) \vdash_\T \r(A) : \m(A) \ra \Type$, and $\mr(\Gamma), x : \m(A), x^* : \r(A) ~x \vdash_\T \m(K) : \Type$. We obtain $\mr(\Gamma) \vdash_\T \Pi x : \m(A). ~\Pi x^* : \r(A) ~x. ~\m(K) : \Type$. 

Suppose that $\Gamma \vdash_\S R : \Pi x : A. ~K$. By induction, we get $\mr(\Gamma), x : \m(A), x^* : \r(A) ~x \vdash_\T \r^{R ~x}(K) : \Kind$. We obtain $\mr(\Gamma) \vdash_\T \Pi x : \m(A). ~\Pi x^* : \r(A) ~x. ~\r^{R ~x}(K) : \Kind$.


\item \underline{\textbf{Abs-Obj}}: By induction, we get $\mr(\Gamma) \vdash_\T \m(A) : \Type$, and $\mr(\Gamma) \vdash_\T \r(A) : \m(A) \ra \Type$, and $\mr(\Gamma), x : \m(A), x^* : \r(A) ~x \vdash_\T \m(B) : \Type$, and $\mr(\Gamma), x : \m(A), x^* : \r(A) ~x \vdash_\T \m(M) : \m(B)$. We derive $\mr(\Gamma) \vdash_\T \lambda x : \m(A). ~\lambda x^* : \r(A) ~x. ~\m(M) : \Pi x : \m(A). ~\Pi x^* : \r(A) ~x. ~\m(B)$.

By induction, we get $\mr(\Gamma), x : \m(A), x^* : \r(A) ~x \vdash_\T \r(B) : \m(B) \ra \Type$ and $\mr(\Gamma), x : \m(A), x^* : \r(A) ~x \vdash_\T \r(M) : \r(B) ~\m(t)$. We derive $\mr(\Gamma) \vdash_\T \lambda x : \m(A). ~\lambda x^* : \r(A) ~x. ~\r(M) : \Pi x : \m(A). ~\Pi x^* : \r(A) ~x. ~\r(B) ~\m(M)$. Using \textsc{Conv-Type}, we obtain $\mr(\Gamma) \vdash_\T \r(\lambda x : A. ~M) : \r(\Pi x : A. ~B) ~\m(\lambda x : A. ~M)$.

\item \underline{\textbf{Abs-Type}}: By induction, we get $\mr(\Gamma) \vdash_\T \m(A) : \Type$, and $\mr(\Gamma) \vdash_\T \r(A) : \m(A) \ra \Type$, and $\mr(\Gamma), x : \m(A), x^* : \r(A) ~x \vdash_\T \m(K) : \Kind$, and $\mr(\Gamma), x : \m(A), x^* : \r(A) ~x \vdash_\T \m(B) : \m(K)$. We derive $\mr(\Gamma) \vdash_\T \lambda x : \m(A). ~\lambda x^* : \r(A) ~x. ~\m(B) : \Pi x : \m(A). ~\Pi x^* : \r(A) ~x. ~\m(K)$.

By induction, we have $\mr(\Gamma), x : \m(A), x^* : \r(A) ~x \vdash_\T \r^{B}(K) : \Kind$ and $\mr(\Gamma), x : \m(A), x^* : \r(A) ~x \vdash_\T \r(B) : \r^{B}(K)$. We derive $\mr(\Gamma) \vdash_\T \lambda x : \m(A). ~\lambda x^* : \r(A) ~x). ~\r(B) : \Pi x : \m(A). ~\Pi x^* : \r(A) ~x. ~\r^{B}(K)$. Using \textsc{Conv-Kind}  and the fact that $\r^{(\lambda x : A. ~B) ~x}(K) \equiv_{\beta\R} \r^{B}(K)$, we obtain $\mr(\Gamma) \vdash_\T \r(\lambda x : A. ~B) : \r^{\lambda x : A. ~B}(\Pi x : A. ~K)$.


\item \underline{\textbf{App-Obj}}: By induction, we have $\mr(\Gamma) \vdash_\T \m(M) : \Pi x : \m(A). ~\Pi x^* : \r(A) ~x. ~\m(B)$, and $\mr(\Gamma) \vdash_\T \m(N) : \m(A)$, and $\mr(\Gamma) \vdash_\T \r(N) : \r(A) ~\m(N)$. We derive $\mr(\Gamma) \vdash_\T \m(M) ~\m(N) ~\r(N) : \m(B)[x \leftarrow \m(N), x^* \leftarrow \r(N)]$. Using \Cref{prop_subst_mr}, we obtain $\mr(\Gamma) \vdash_\T \m(M ~N) : \m(B[x \leftarrow N])$.

By induction, we get $\mr(\Gamma) \vdash_\T \r(M) : \Pi x : \m(A). ~\Pi x^* : \r(A) ~x. ~\r(B) ~(\m(M) ~x ~x^*)$. It follows that $\mr(\Gamma) \vdash_\T \r(M) ~\m(N) ~\r(N) : \r(B)[x \leftarrow \m(N), x^* \leftarrow \r(N)] ~(\m(M) ~\m(N) ~\r(N))$. Using \Cref{prop_subst_mr}, we obtain $\mr(\Gamma) \vdash_\T \r(M ~N) : \r(B[x \leftarrow N]) ~\m(M ~N)$.


\item \underline{\textbf{App-Type}}: By induction, we have $\mr(\Gamma) \vdash_\T \m(A) : \Pi x : \m(B). ~\Pi x^* : \r(B) ~x. ~\m(K)$, and $\mr(\Gamma) \vdash_\T \m(M) : \m(B)$, and $\mr(\Gamma) \vdash_\T \r(M) : \r(B) ~\m(M)$. We derive $\mr(\Gamma) \vdash_\T \m(A) ~\m(M) ~\r(M) : \m(K)[x \leftarrow \m(M), x^* \leftarrow \r(M)]$. Using \Cref{prop_subst_mr}, we obtain $\mr(\Gamma) \vdash_\T \m(A ~M) : \m(K[x \leftarrow M])$.


By induction, we get $\mr(\Gamma) \vdash_\T \r(A) : \Pi x : \m(B). ~\Pi x^* : \r(B) ~x. ~\r^{A ~x}(K)$. It follows that $\mr(\Gamma) \vdash_\T \r(A) ~\m(M) ~\r(M) : \r^{A ~x}(K)[x \leftarrow \m(M), x^* \leftarrow \r(M)]$. Using \Cref{prop_subst_mr}, we obtain $\mr(\Gamma) \vdash_\T \r(A ~M) : \r^{A ~M}(K[x \leftarrow M])$.


\item \underline{\textbf{Conv-Type}}: By induction, we get $\mr(\Gamma) \vdash_\T \m(M) : \m(A)$, and $\mr(\Gamma) \vdash_\T \r(M) : \r(A) ~\m(M)$, and $\mr(\Gamma) \vdash_\T \m(B) : \Type$, and $\mr(\Gamma) \vdash_\T \r(B) : \m(B) \ra \Type$. Since $A \equiv_{\beta\R} B$ in $\S$, we have $\m(A) \equiv_{\beta\R} \m(B)$ and $\r(A) \equiv_{\beta\R} \r(B)$ in $\T$ using \Cref{prop_conv_mr}. We derive $\mr(\Gamma) \vdash_\T \m(M) : \m(B)$ and $\mr(\Gamma) \vdash_\T \r(M) : \r(B) ~\m(M)$.


\item \underline{\textbf{Conv-Kind}}: By induction, we get $\mr(\Gamma) \vdash_\T \m(A) : \m(K)$, and $\mr(\Gamma) \vdash_\T \r(A) : \r^{A}(K)$, and $\mr(\Gamma) \vdash_\T \m(K') : \Kind$, and $\mr(\Gamma) \vdash_\T \r^{A}(K') : \Kind$. Since $K \equiv_{\beta\R} K'$ in $\S$, we have $\m(K) \equiv_{\beta\R} \m(K')$ and $\r^{A}(K) \equiv_{\beta\R} \r^{A}(K')$ in $\T$ using \Cref{prop_conv_mr}. We derive $\mr(\Gamma) \vdash_\T \m(A) : \m(K')$ and $\mr(\Gamma) \vdash_\T \r(A) : \r^{A}(K')$.
\end{itemize}
\end{proof}




\subsection{Example: Natural Numbers and Integers}


The theory of natural numbers can be embedded into the theory of integers using this new translation template. We need to set the parameters of the theory of natural numbers.

We give here the intuition on how to find the parameters for the encoding of the Calculus of Constructions. If $a : \Set$, we want $\m(a) : \Set$ and $\r(a) : \El ~\m(a) \ra \El ~\o$, where $\r(a)$ is a predicate asserting that an object of type $\El ~\m(a)$ indeed corresponds to an object of type $\El ~a$. If $t : \El ~a$, we want $\m(t) : \El ~\m(a)$ and $\r(t) : \Prf ~(\r(a) ~\m(t))$, where $\r(t)$ is a proof that $\m(t)$ satisfies $\r(a)$.
%%%
\begin{flalign*}
&\m(\Set) = \Set & \\
&\r(\Set) = \lambda x : \Set. ~\El ~x \ra \El ~\o & \\
&\m(\El) = \lambda x : \Set. ~\lambda x^* : \El ~x \ra \El ~\o. ~\El ~x & \\
&\r(\El) = \lambda x : \Set. ~\lambda x^* : \El ~x \ra \El ~\o. ~\lambda z : \El ~x. ~\Prf ~(x^* ~z) & 
\end{flalign*}
%%%
If we have a proposition $p : \El ~\o$, we want $\m(p) : \El ~\o$. It follows that $\m(p)$ is indeed a proposition, hence we define $\r(\o)$ so that we always have an inhabitant $\r(p)$ of type $\Prf ~(\r(\o) ~p)$. A proof $h : \Prf ~p$ is mapped to a proof $\m(h) : \Prf ~\m(p)$. Since $\m(h)$ is indeed a proposition, we encode $\r(\Prf)$ so that we always have an inhabitant $\r(h)$ of type $\r(\Prf ~p) ~m(h)$.
%%%
\begin{flalign*}
&\m(\Prf) = \lambda x : \El ~\o. ~\lambda x^* : \Prf ~(\r(\o) ~x). ~\Prf ~x & \\
&\r(\Prf) = \lambda x : \El~\o. ~\lambda x^* : \Prf ~(\r(\o) ~x). ~\lambda z : \Prf ~x. ~\Prf ~x & \\
&\m(\o) = \o & \\
&\r(\o) = \lambda z : \El ~\o. ~z \impd (\lambda x : \Prf ~z. ~z) &
\end{flalign*}
%%%
The parameters for $\arrd$, $\impd$, $\pi$ and $\fa$ are defined so that the conditions on the rewrite rules are satisfied. For instance, we set 
%%%
\[
\begin{array}{ll}
\m(\impd) = &\lambda a : \El ~\o. ~\lambda a^* : \Prf ~(\r(\o) ~a). ~\lambda b : \Pi x : \Prf ~a. ~\Prf ~a \ra \El ~\o. \\
&\lambda b^* : \Pi x : \Prf ~a. ~\Pi x^* : \Prf ~a. ~\Prf ~(\r(\o) ~(b ~x ~x^*)). \\
&a \impd (\lambda x : \Prf ~a. ~a \impd ~(b ~x)) \\
\end{array}
\]
%%%
because the theory embedding requires $\m(\Prf ~(a \impd b)) \equiv_{\beta\Sigma} \m(\Pi z : \Prf ~a. ~\Prf ~(b ~z))$. 

The sort of natural numbers is embedded into the sort of integers using the predicate $\r(\nat)$ asserting that an integer is non-negative. The parameters for $0$ and $\succ$ are immediate: $\r(0)$ is a proof term of $\Prf ~(0 \geq 0)$ and $\r(\succ)$ is a proof of $\Pi x : \El ~\int. ~\Pi x^* : \Prf ~(x \geq 0). ~\Prf ~(\succ ~x \geq x)$.
%%%
\begin{flalign*}
&\m(\nat) = \int & \\
&\r(\nat) = \lambda z : \El ~\int. ~z \geq 0 & \\
&\m(0) = 0 & \\
&\r(0) = \ax_1 ~0 & \\
&\m(\succ) = \lambda x : \El ~\int. ~\lambda x^* : \Prf ~(x \geq 0). ~\succ ~x & \\
&\r(\succ) = \lambda x : \El ~\int. ~\lambda x^* : \Prf ~(x \geq 0). ~\ax_3 ~(\succ ~x) ~x ~0 ~(\ax_2 ~x) ~x^* & \\
&\m(\geq) = \lambda x. ~\lambda x^*. ~\lambda y. ~\lambda y^*. ~\geq ~x ~y & \\
&\r(\geq) = \lambda x. ~\lambda x^*. ~\lambda y. ~\lambda y^*. ~\lambda p. ~p & \\
&\m(\ax_1) = \lambda x. ~\lambda x^*. ~\ax_1 ~x & \\
&\r(\ax_1) = \m(\ax_1) & 
\end{flalign*}
%%%
The parameters $\m(\geq)$ and $\m(\ax_1)$ are intuitive. Following the definitions of $\r(\o)$ and $\r(\Prf)$, the parameters $\r(\geq)$ and $\r(\ax_1)$ do not bring any relevant invariant.

All the remaining parameters are given in~\cite{deduktinterp} and have been implemented in \dk. In particular, the parameter $\m(\rec)$ requires proof irrelevance---the principle stating that two proofs of a same proposition are equal.



\subsection{From Sorted Logic to Unsorted Logic}


In \lpr, we encode sorted logic using the universe of sorts $\Set$ and the injection $\El$ that maps any sort to the type of its elements. 
%%%
\begin{flalign*}
&\Set : \Type &
&\El : \Set \ra \Type &
&\Prop : \Type &
&\Prf : \Prop \ra \Type 
\end{flalign*} 
%%%
It follows that objects have type $\El ~a$, for some sort $a$. 
We consider here sorted logic with dependent implication and universal quantifier. 
The semantic of both connectives is given by constants representing their natural deduction rules.
%%%
\begin{flalign*}
&\impd : \Pi p : \Prop. ~(\Prf ~p \ra \Prop) \ra \Prop & \\
&\mathsf{impd_i} : \Pi p : \Prop. ~\Pi q : \Prf ~p \ra \Prop. ~(\Pi z : \Prf ~p. ~\Prf ~(q ~z)) \ra \Prf ~(p \impd q) & \\
&\mathsf{impd_e} : \Pi p : \Prop. ~\Pi q : \Prf ~p \ra \Prop. ~\Prf ~(p \impd q) \ra \Pi z : \Prf ~p. ~\Prf ~(q ~z) & \\
&\fa : \Pi a : \Set. ~(\El ~a \ra \Prop) \ra \Prop & \\
&\mathsf{all_i} : \Pi a : \Set. ~\Pi p : \El ~a \ra \Prop. ~(\Pi x : \El ~a. ~\Prf ~(p ~x)) \ra \Prf ~(\fa ~a ~p) & \\
&\mathsf{all_e} : \Pi a : \Set. ~\Pi p : \El ~a \ra \Prop. ~\Prf ~(\fa ~a ~p) \ra \Pi x : \El ~a. ~\Prf ~(p ~x) & 
\end{flalign*}
%%%
In unsorted logic, objects do not have type $\El ~a$ anymore, but have the generic type $\tm$.
%%%
\begin{flalign*}
&\tm : \Type & 
&\Prop : \Type & 
&\Prf : \Prop \ra \Type
\end{flalign*} 
%%%
The connectives are encoded similarly than in sorted logic, except that the universal quantifier is not polymorphic anymore, as we do not have sorts.
%%%
\begin{flalign*}
&\impd : \Pi p : \Prop. ~(\Prf ~p \ra \Prop) \ra \Prop & \\
&\mathsf{impd_i} : \Pi p : \Prop. ~\Pi q : \Prf ~p \ra \Prop. ~(\Pi z : \Prf ~p. ~\Prf ~(q ~z)) \ra \Prf ~(p \impd q) &\\
&\mathsf{impd_e} : \Pi p : \Prop. ~\Pi q : \Prf ~p \ra \Prop. ~\Prf ~(p \impd q) \ra \Pi z : \Prf ~p. ~\Prf ~(q ~z) & \\
&\fa : (\tm \ra \Prop) \ra \Prop & \\
&\mathsf{all_i} : \Pi p : \tm \ra \Prop. ~(\Pi x : \tm. ~\Prf ~(p ~x)) \ra \Prf ~(\fa ~p) & \\
&\mathsf{all_e} : \Pi p : \tm \ra \Prop. ~\Prf ~(\fa ~p) \ra \Pi x : \tm. ~\Prf ~(p ~x) & 
\end{flalign*}
%%%
One way to translate sorted logic into unsorted logic is to represent sorts in unsorted logic using predicates. 
For example, instead of having objects of type $\El ~a$, we have objects of type $\tm$ but which satisfy the sort predicate corresponding to the sort $a$. 

Theory embeddings are well suited to embedding sorted logic into unsorted logic, as this translation template allows us to introduce predicates.
The key of the translation is the insertion of sort predicates using $\r(\El)$. For some symbols, the parameter $\r$ is not relevant, but the translation requires such parameters. 
We introduce $\unit$ of type $\Type$ and $\star$ of type $\unit$, so that we can give $\star$ as a witness of $\unit$.  
%%%
\begin{flalign*}
&\m(\Set) = \unit & \\
&\r(\Set) = \lambda z : \unit. ~\tm \ra \Prop & \\
&\m(\El) = \lambda x : \unit. ~\lambda x^* : \tm \ra \Prop. ~\tm & \\
&\r(\El) = \lambda x : \unit. ~\lambda x^* : \tm \ra \Prop. ~\lambda z : \tm. ~\Prf ~(x^* ~z) & \\
&\m(\Prop) = \Prop & \\
&\r(\Prop) = \lambda p : \Prop. ~\unit & \\
&\m(\Prf) = \lambda p : \Prop. ~\lambda p^* : \unit. ~\Prf ~p & \\
&\r(\Prf) = \lambda p : \Prop. ~\lambda p^* : \unit. ~\lambda z : \Prf ~p. ~\unit & 
\end{flalign*} 
%%%
The connectives $\impd$ and $\fa$ are set consequently. 
In particular, the polymorphic quantifier of sorted logic is mapped to the generic quantifier of unsorted logic, but the sort information is stored inside the predicate.
%%%
\begin{flalign*} 
&\m(\impd) = \lambda p. ~\lambda p^*. ~\lambda q. ~\lambda q^*. ~p \impd (\lambda z : \Prf ~p. ~q ~z ~\star) & \\
&\r(\impd) = \lambda p. ~\lambda p^*. ~\lambda q. ~\lambda q^*. ~\star & \\
&\m(\fa) = \lambda a. ~\lambda a^*. ~\lambda p. ~\lambda p^*. ~\fa ~(\lambda x : \tm. ~(a^* ~x) \impd (p ~x)) & \\
&\r(\fa) = \lambda a. ~\lambda a^*. ~\lambda p. ~\lambda p^*. ~\star & 
\end{flalign*} 
%%%
The parameter $\m(\mathsf{impd_i})$ is built using the constant $\mathsf{impd_i}$ of the unsorted encoding. We take
\[
\begin{array}{ll}
\m(\mathsf{impd_i}) = &\lambda p : \Prop. ~\lambda p^* : \unit. \\
&\lambda q : (\Pi z : \Prf ~p. ~\Pi z^* : \unit. ~\Prop). \\
&\lambda q^* : (\Pi z : \Prf ~p. ~\Pi z^* : \unit. ~\unit). \\
&\lambda h : (\Pi z : \Prf ~p. ~\Pi z^* : \unit. ~\Prf ~(q ~z ~z^*)). \\
&\lambda h^* : (\Pi z : \Prf ~p. ~\Pi z^* : \unit. ~\unit). \\
&\mathsf{impd_i} ~p ~(\lambda z : \Prf ~p. ~q ~z ~\star) ~(\lambda z : \Prf ~p. ~h ~z ~\star)
\end{array}
\]
which indeed returns a proof of $\m(p \impd q)$. 
We can do the same for the constants representing the other natural deduction rules. 
For $\m(\mathsf{impd_e})$, we need an additional axiom stating that two inhabitants of $\unit$ are interchangeable---just like we had to assume proof irrelevance in the example of natural numbers and integers.


SOLUTION WITH PAIRS


The natural idea is to apply a theory morphism, where any term of type $\El ~a$ is mapped to a pair containing a term of type $\tm$ and a proof that this term satisfies the predicate associated to $a$. 

As a preliminary step, we encode dependent pairs in \lpr. 
Pairs are built via the constructor $\mathsf{mk\_pair}$, and the elements of pairs are accessible via $\mathsf{fst}$ and $\mathsf{snd}$. 
The semantic of $\mathsf{fst}$, $\mathsf{snd}$ and $\mathsf{mk\_pair}$ is given via rewrite rules.
%%%
\begin{flalign*}
&\mathsf{pair} : (\tm \ra \Prop) \ra \Type & \\
&\mathsf{mk\_pair} : \Pi p : (\tm \ra \Prop). ~\Pi t : \tm. ~\Prf ~(p ~t) \ra \mathsf{pair} ~p & \\
&\mathsf{fst} : \Pi p : (\tm \ra \Prop). ~\Pi m : \mathsf{pair} ~p. ~\tm & \\
&\mathsf{snd} : \Pi p : (\tm \ra \Prop). ~\Pi m : \mathsf{pair} ~p. ~\Prf ~(p ~(\mathsf{fst} ~p ~m)) & \\
&\mathsf{fst} ~p ~(\mathsf{mk\_pair} ~p ~t ~h) \lra t & \\
&\mathsf{snd} ~p ~(\mathsf{mk\_pair} ~p ~t ~h) \lra h & \\
&\mathsf{mk\_pair} ~p ~(\mathsf{fst} ~p ~m) ~(\mathsf{snd} ~p ~m) \lra m &
\end{flalign*} 
%%%
We define $\mor(Set)$ so that sorts $a$ are mapped to predicates of type $\tm \ra \Prop$, and we define $\mor(\El)$ so that terms of type $\El ~a$ are mapped to pairs of type $\mathsf{pair} ~\mor(a)$.
%%%
\begin{flalign*}
&\mor(\Set) = \tm \ra \Prop & \\
&\mor(\El) = \lambda p : \tm \ra \Prop. ~\mathsf{pair} ~p & \\
&\mor(\Prop) = \Prop & \\
&\mor(\Prf) = \Prf &
\end{flalign*} 
%%%
Sorts do not occur in the types of $\impd$, $\mathsf{impd_i}$ and $\mathsf{impd_e}$, so the parameters $\mor(\impd)$, $\mor(\mathsf{impd_i})$ and $\mor(\mathsf{impd_e})$ are straightforward. 
The polymorphic quantifier of sorted logic is mapped to the generic quantifier of unsorted logic, but the sort information is stored inside the predicate.
%%%
\begin{flalign*}
&\mor(\impd) = \impd & \\
&\mor(\mathsf{impd_i}) = \mathsf{impd_i} & \\
&\mor(\mathsf{impd_e}) = \mathsf{impd_e} & \\
&\mor(\fa) = \lambda a. ~\lambda p. ~\fa ~(\lambda x : \tm. ~(a ~x) \impd (\lambda h. ~p ~(\mathsf{mk\_pair} ~a ~x ~h))) & 
\end{flalign*}
%%%
Remark that it is important to have a \textit{dependent} implication $\impd$ instead of an usual implication $\imp$ in the definition of the parameter $\mor(\fa)$. 

It remains to define the parameter $\mor(\mathsf{all_i})$.
%%%
\[
\begin{array}{ll}
\mor(\mathsf{all_i}) = & \lambda a : \tm \ra \Prop. ~\lambda p : \mathsf{pair} ~a \ra \Prop. \\
&\lambda H : \Pi m : \mathsf{pair} ~a. ~\Prf ~(p ~m). \\
& \mathsf{all_i} \\
&\hspace{0.5cm} (\lambda x. ~(a ~x) \impd (\lambda h. ~p ~(\mathsf{mk\_pair} ~a ~x ~h))) \\
&\hspace{0.5cm} (\lambda x. ~\mathsf{impd_i} ~(a ~x) \\
&\hspace{1cm} (\lambda h. ~p ~(\mathsf{mk\_pair} ~a ~x ~h)) \\
&\hspace{1cm} (\lambda h. ~H ~(\mathsf{mk\_pair} ~a ~x ~h)))
\end{array}
\]
%%%
The dependent pairs introduced by this theory morphism can be erased. We could have used a theory embedding, but such translation template artificially inserts invariants even when they are not needed. 
By introducing dependent pairs through the theory morphism and later erase the dependent pairs, we only insert invariants when they are needed.


